Tensorformer: Normalized Matrix Attention Transformer for High-quality Point Cloud Reconstruction

Surface reconstruction from raw point clouds has been studied for decades in the computer graphics community, which is highly demanded by modeling and rendering applications nowadays. Classic solutions, such as Poisson surface reconstruction, require point normals as extra input to perform reasonable results. Modern transformer-based methods can work without normals, while the results are less fine-grained due to limited encoding performance in local fusion from discrete points. We introduce a novel normalized matrix attention transformer (Tensorformer) to perform high-quality reconstruction. The proposed matrix attention allows for simultaneous point-wise and channel-wise message passing, while the previous vector attention loses neighbor point information across different channels. It brings more degree of freedom in feature learning and thus facilitates better modeling of local geometries. Our method achieves state-of-the-art on two commonly used datasets, ShapeNetCore and ABC, and attains 4% improvements on IOU on ShapeNet. Code can be accessed https://github.com/THHHomas/Tensorformer6.

==> figures/ablation.tex <==
\begin{figure} 
\centering
  \includegraphics[width=\columnwidth,height=\columnwidth]{figures/images/ablation}
  \caption{Evaluation of the effectiveness of the two mechanisms, matrix attention and weight normalization, on airplane, bench and vessel. For detailed analysis, please refer to the text.}
  \label{fig:ab}
\end{figure}

% \begin{figure} 
%   \includegraphics[width=\columnwidth]{figures/images/ablation2.PNG}
%   \caption{This figure shows the effectiveness of the two mechanisms we proposed on vessel.}
%   \label{fig:ab2}
% \end{figure}
% \begin{figure} 
%   \includegraphics[width=\columnwidth]{figures/images/ablation3.PNG}
%   \caption{This figure shows the effectiveness of the two mechanisms we proposed on bench.}
%   \label{fig:ab3}
% \end{figure}


==> figures/ablation_all.tex <==
\begin{figure} 
\centering
  \includegraphics[width=\columnwidth]{figures/images/ablation_all}
  \caption{Evaluation of the effectiveness of the two mechanisms, matrix attention and weight normalization, on 13 categories.}
  \label{fig:ab_all}
\end{figure}

==> figures/conv.tex <==
\begin{figure}
\centering
  \includegraphics[width=0.75\columnwidth]{figures/images/conv}
  \caption{Consider a convolution operator with kernel size $W\times H$, the feature channel in layer 0 is $C$, then every cube in layer 1 merge the information from $W\times H\times C$ cubes. A cube represent one value in feature.
}
  \label{fig:conv}
\end{figure}

==> figures/g2.tex <==


\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/g2}
  \caption{Generalization results. The first column is input point cloud. The second column is the results training on vessel and testing on airplane. The third column is the ground-truth. The fourth column is input point cloud. The fifth column is the results training on airplane and testing on vessel. The sixth column is the ground-truth}
  \label{fig:g2}
  
  
\end{figure*}

==> figures/main_result2.tex <==
\begin{figure*} 
\centering
  \includegraphics[width=2\columnwidth]{figures/images/main_result2}
  \caption{Visualized results of our method and 2 traditional reconstruction methods PSR and BPA.}
  \label{fig:main_result2}
\end{figure*}
